The Cosmic Ultraviolet Baryon Survey (CUBS) IV: The Complex Multiphase Circumgalactic Medium as Revealed by Partial Lyman Limit Systems

We present a detailed study of two partial Lyman limit systems (pLLSs) of neutral hydrogen column density $N_\mathrm{H\,I}\approx(1-3)\times10^{16}\,\mathrm{cm}^{-2}$ discovered at $z=0.5$ in the Cosmic Ultraviolet Baryon Survey (CUBS). Available far-ultraviolet spectra from the Hubble Space Telescope Cosmic Origins Spectrograph and optical echelle spectra from MIKE on the Magellan Telescopes enable a comprehensive ionization analysis of diffuse circumgalactic gas based on resolved kinematics and abundance ratios of atomic species spanning five different ionization stages. These data provide unambiguous evidence of kinematically aligned multi-phase gas that masquerades as a single-phase structure and can only be resolved by simultaneous accounting of the full range of observed ionic species. Both systems are resolved into multiple components with inferred $\alpha$-element abundance varying from $[\alpha/\text{H}]\approx\!{-0.8}$ to near solar and densities spanning over two decades from $\log n_\mathrm{H}\mathrm{cm}^{-3}\approx\!-2.2$ to $<-4.3$. Available deep galaxy survey data from the CUBS program taken with VLT/MUSE, Magellan/LDSS3-C and Magellan/IMACS reveal that the $z=0.47$ system is located 55 kpc from a star-forming galaxy with prominent Balmer absorption of stellar mass $M_\star\approx2\times10^{10}M_\odot$, while the $z=0.54$ system resides in an over-dense environment of 11 galaxies within 750 kpc in projected distance, with the most massive being a luminous red galaxy of $M_\star\approx2\times10^{11}M_\odot$ at 375 kpc. The study of these two pLLSs adds to an emerging picture of the complex, multiphase circumgalactic gas that varies in chemical abundances and density on small spatial scales in diverse galaxy environments. The inhomogeneous nature of metal enrichment and density revealed in observations must be taken into account in theoretical models of diffuse halo gas.

==> figures/abundances_table.tex <==
\begin{table*}
\begin{tabular}{lRRRRRRR}
\caption{Summary of density and chemical abundance inferences for individual components$^a$\label{table:abundances}}
\colhead{} & \nocolhead{$\Delta v\tablenotemark{b}$} & \nocolhead{$\log\N{H\,I}/\cmx{-2}$} & \colhead{$\log\nH/\cmx{-3}$} & \colhead{[$\alpha$/H]} & \colhead{[C/H]} & \colhead{[N/H]} & \colhead{[Fe/H]} &\colhead{[C/$\alpha]$} & \colhead{[N/$\alpha]$}}
\hline
$z=0.47$ c1L & \xpm{-2.28}{+0.14}{-0.07} & \xpm{-0.81}{+0.06}{-0.05} & -0.66\pm0.10    & <-0.58 & <-0.06 & 0.14\pm0.10 & <0.28\\
$z=0.47$ c1H & \xpm{-3.51}{+0.11}{-0.14} & >-0.94 & <0.6 & <0.5  & \nodata & <-0.33 & \nodata \\
$z=0.47$ c2 & -2.38\pm0.13 & -0.12\pm0.11 & 0.14\pm0.11 & <0.31 & \nodata & \xpm{0.27}{+0.11}{-0.13} & <0.50\\
$z=0.47$ c3 & -3.77\pm0.05 & -0.07_{-0.13}^{+0.12}& -1.15\pm0.24 & -0.01_{-0.11}^{+0.12}  & \nodata & \xpm{-1.07}{+0.23}{-0.22} & 0.06\pm0.07 \\
$z=0.47$ c4L & -2.67\pm0.11          & 0.08\pm0.05          & 0.41\pm0.14 & 0.30_{-0.15}^{+0.10}    & \nodata & 0.33\pm0.14 & \xpm{0.23}{+0.10}{-0.16}\\
$z=0.47$ c4H & \xpm{-3.85}{+0.15}{-0.13} & >-1.19 & >-1.42 & >-1.40  & \nodata & \xpm{-0.28}{+0.18}{-0.17} & \xpm{0.00}{+0.20}{-0.21} \\
$z=0.47$ c5$^c$ & \nodata & <-0.43 & <-0.14 & <0.51 & \nodata &\nodata &\nodata\\
$z=0.47$ c6$^c$ & \nodata &<0.48 & <0.41 & \nodata & \nodata &\nodata & \nodata\\
\hline\hline
$z=0.54$ c1L & \xpm{-2.56}{+0.10}{-0.08} & -0.12\pm0.06 & \xpm{-0.26}{+0.20}{-0.24} & \xpm{-0.17}{+0.09}{-0.10} & 0.09\pm0.11 & \xpm{-0.15}{+0.20}{-0.23} & \xpm{-0.05}{+0.10}{-0.11}\\
$z=0.54$ c1H & <-2.97 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata\\
$z=0.54$ c2 &-3.37_{-0.14}^{+0.13} & -0.03_{-0.21}^{+0.19} & >-1.2 & 0.44\pm0.24  & \nodata & >-1.04 & \xpm{0.50}{+0.19}{-0.21}\\
$z=0.54$ c3 & <-4.33 & <-0.77 & <-1.22 & <-1.22 & \nodata& \nodata& \nodata \\
% \tablenotetext{a}{Errors represent 68\% credible intervals.}
% \tablenotetext{b}{$\Delta v$ is given in units of \kms.}
% \tablenotetext{c}{For components without detected metals, abundance limits are obtained assuming $-5\leq n_\mathrm{H}\leq-2$.}
\end{tabular
\end{table*}
